The Evolution of Compact Binary Star Systems

We review the formation and evolution of compact binary stars consisting of white dwarfs (WDs), neutron stars (NSs), and black holes (BHs). Mergings of compact binary stars are expected to be the most important sources for the forthcoming gravitational-wave (GW) astronomy. In the first part of the review, we discuss observational manifestations of close binary stars with NS and/or black components and their merger rate, crucial points in the formation and evolution of compact stars in binary systems, including the treatment of the natal kicks which NSs and BHs acquire during the core collapse of massive stars and the common envelope phase of binary evolution, which are most relevant to the merging rates of NS-NS, NS-BH and BH-BH binaries. The second part of the review is devoted mainly to formation and evolution of binary WDs and their observational manifestations, including their role as progenitors of cosmologically important thermonuclear SN Ia. We also consider AM CVn-stars which are thought to be the best verification binary GW sources for future low-frequency GW space interferometers.

==> new_formation_DCB3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Formation of Double Compact Binaries}
%\label{section:binary_NS}

%%%% revised by KP may 2013


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Analytical estimates}

A rough estimate of the formation rate of double compact binaries can
be obtained ignoring many details of binary evolution. To do this, we
shall use the observed initial distribution of binary orbital
parameters and assume the simplest conservative mass transfer
($M_1 + M_2= \mathrm{const}$) without kick velocity imparted to the
nascent compact stellar remnants during SN explosions.

\paragraph*{Initial binary distributions.}
From observations of spectroscopic binaries it is possible to derive
the formation rate of binary stars with initial masses $M_1$, $M_2$
(with mass ratio $q=M_2/M_1\le 1$), orbital semimajor axis $A$, and
eccentricity $e$. According to~\cite{Popova_al82}, the present
birth rate of binaries in our Galaxy can be written in factorised
form as 
%
\begin{equation}
  \frac{dN}{dA\,dM_1\,dq\,dt} \approx
  0.087 \left( \frac{A}{R_\odot} \right)^{-1}
  \left( \frac{M_1}{M_\odot} \right)^{-2.5} f(q),
  \label{E:bin_brate}
\end{equation}
%
where $f(q)$ is a poorly constrained distribution over the initial mass
ratio of binary components.

One usually assumes a mass ratio distribution law in the form 
$f(q)\sim q^{-\alpha_q}$ where $\alpha_q$ is a
free parameter; another often used form of the $q$-distribution was
suggested by Kuiper~\cite{Kuiper35}:
%
\begin{displaymath}
  f(q) = 2/(1+q)^2.
\end{displaymath} 
%
The range of $A$ is $10 \leq A/R_\odot \leq 10^6$. In deriving the above
Eq.~(\ref{E:bin_brate}), Popova et al.~\cite{Popova_al82} took
into account selection effects to convert the ``observed'' distribution of
stars into the true one. An almost flat logarithmic distribution of
semimajor axes was also found in~\cite{Abt83}. 

\textbf{Taken at face value, assuming 100\% binarity, mass limits of the primary component $M_1=0.08 M_\odot$  to $100 M_\odot$, a flat distribution over semimajor axes 
(contact at ZAMS)$<\log (A/R_\odot)<$~(border between close and wide binaries), $f(q)=1$ 
for close binaries, and $f(q)\propto q^{-2.5}$ for $0.3\leq q \leq 1$ and  $f(q)=2.14$ 
for $q<0.3$ for wide binaries with $\log(A/R_\odot)\leq 6$,
as accepted in Tutukov and Yungelson's BPS code \emph{IBiS}, 
we get SFR~$\approx 8 M_\odot$ per yr, which is several times as high as the
currently estimated present-day Galactic SFR. If 8 $M_\odot$ per year 
is used as a constant average SFR for 13.5~Gyr, we get the right mass of the Galactic disc. 
Clearly, this estimate is rather formal, since most of the stellar  
mass resides in low-mass stars for which IMF, $f(q)$, $f(A)$, the binary fraction, etc., 
are poorly known. However, if we consider only  
stars with $M_1>0.95 M_\odot$ (which can evolve off the main sequence in the Hubble time), we get, under the  ``standard'' assumptions in the \emph{IBiS} code, 
e. g., a WD formation rate of 0.65 per yr, which is reasonably 
consistent with observational estimates (e. g., Liebert et al. \cite{2005ApJS..156...47L}), 
the SNII+SNIb/c rate about 1.5/100 per yr, which is consistent with the inferred Galactic rate 
(e. g. Cappellaro \cite{2001MmSAI..72..863C}) or with the pulsar formation rate 
(e. g., Vranesevic et al. \cite{2004ApJ...617L.139V}). We also get the proper rate of WD+WD mergers for SN Ia (a few per thousand years).}        

%Integration of
%Eq.~(\ref{E:bin_brate}) yields one binary system with $M_1\gtrsim
%0.8M_\odot$ and $10\,R_\odot < A < 10^6\,R_\odot$ per year in the
%Galaxy.  which is in reasonable agreement with the Galactic star
%formation rate estimated by various methods; the present-day star
%formation rate is \textbf{a few $M_\odot$ per year (see, e.g., \cite{2011AJ....142..197C,2012ARAA..50..531K,2013ASSP...34...29N})}.

\paragraph*{Constraints from conservative evolution.}
To form a NS at the end of thermonuclear evolution, in this estimate we shall
assume that the primary mass
should be at least $10\,M_\odot$. Eq.~(\ref{E:bin_brate}) says
that the formation rate of such binaries is about 1 per 50 years. We
shall restrict ourselves by considering only close binaries, in which
mass transfer onto the secondary is possible. This narrows the binary
separation interval to $10\mbox{\,--\,}1000\,R_\odot$ (see
Figure~\ref{f:remn}); the birth rate of close massive
($M_1>10\,M_\odot$) binaries is thus $1/50 \times 2/5 \mathrm{\ yr}^{-1} =
1/125 \mathrm{\ yr}^{-1}$. The mass ratio $q$ should not be very small
to make the formation of the second NS possible. The lower limit for $q$ is
derived from the condition that after the first mass transfer stage,
during which the mass of the secondary increases, $M_2+\Delta M\ge
10\,M_\odot$. Here $\Delta M=M_1-M_{\mathrm{He}}$ and the mass of the helium
core left after the first mass transfer is $M_{\mathrm{He}}\approx 0.1
(M_1/M_\odot)^{1.4}$. This yields
%
\begin{displaymath}
  m_2+(m_1-0.1m_1^{1.4}) > 10,
\end{displaymath}
%
where we used the notation $m=M/M_\odot$, or in terms of $q$:
%
\begin{equation}
  q \ge 10/m_1+0.1 m_1^{0.4}-1.
  \label{E:ll_q}
\end{equation}

An upper limit for the mass ratio is obtained from the requirement
that the binary system remains bound after the sudden mass loss in the
second supernova explosion\epubtkFootnote{For the first supernova
  explosion without kick this is always satisfied.}. From
Eq.~(\ref{A:SN:symm-ecc}) we obtain
%
\begin{displaymath}
  \frac{0.1[m_2+(m_1-0.1m_1^{1.4})]^{1.4}-1.4}{2.8} < 1,
\end{displaymath}
%
or in terms of $q$:
%
\begin{equation}
  q \le 14.4/m_1+0.1m_1^{0.4}-1.
  \label{E:ul_q}
\end{equation}

Inserting $m_1=10$ in the above two equations yields the appropriate
mass ratio range $0.25< q< 0.69$, i.e.\ 20\% of the binaries for Kuiper's
mass ratio distribution. So we conclude that the birth rate of binaries
which potentially can produce double NS system is $\lesssim 0.2 \times
1/125 \mathrm{\ yr}^{-1} \simeq 1/600 \mathrm{\ yr}^{-1}$.

Of course, this is a very crude upper limit -- we have not taken into
account the evolution of the binary separation, ignored initial binary
eccentricities, non-conservative mass loss, etc. However, it is not
easy to treat all these factors without additional knowledge of
numerous details and parameters of binary evolution (such as the
physical state of the star at the moment of the Roche lobe overflow,
the common envelope efficiency, etc.). All these factors should
decrease the formation rate of double NS. The coalescence rate of
compact binaries (which is ultimately of interest for us) will be even
smaller -- for the compact binary to merge within the Hubble time, the
binary separation after the second supernova explosion should be less
than $\sim 100\,R_\odot$ (orbital periods shorter than $\sim$~40~d) 
for arbitrary high orbital eccentricity $e$ (see Figure~\ref{A:GW:p-e}).
The model-dependent distribution of NS kick velocities provides another
strong complication. We also stress that this upper limit was obtained
assuming a constant Galactic star-formation rate and normalisation 
of the binary formation by Eq.~(\ref{E:bin_brate}).

Further (semi-)analytical investigations of the parameter space of binaries
leading to the formation of coalescing binary NSs are still possible
but technically very difficult, and we shall not reproduce them here.
The detailed semi-analytical approach to the problem of formation of NSs in
binaries and evolution of compact binaries has been developed by Tutukov and
Yungelson~\cite{Tutukov_Yungelson93a, ty93b}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Population synthesis results}

A distinct approach to the analysis of binary star evolution is based
on the population synthesis method -- a Monte Carlo simulation of the
evolution of a sample of binaries with different initial
parameters. 
This approach was first applied to model various
observational manifestations of magnetized NSs in massive binary
systems~\cite{Kornilov_Lipunov83a, Kornilov_Lipunov83b,
  Dewey_Cordes87} and generalised to binary systems of arbitrary mass
in~\cite{Lipunov_al96} (The Scenario Machine code). To achieve a
sufficient statistical significance, such simulations usually involve
a large number of binaries, typically of the order of a million. The
total number of stars in the Galaxy is still four orders of magnitude
larger, so this approach cannot guarantee that rare stages of the
binary evolution will be adequately reproduced\epubtkFootnote{Instead
  of Monte Carlo simulations one may use a sufficiently dense grid in
  the 3D space of binary parameters and integrate over this grid (see,
  e.g., \cite{ty02} and references therein).}.

Presently, there are several population synthesis codes used for
massive binary system studies, which take into account with different
degree of completeness various aspects of binary stellar evolution
(e.g., the codes by Portegies Zwart et
al.~\cite{py98, yungelson_bh06}, Bethe and
Brown~\cite{Bethe_Brown98}, Hurley, Tout, and Pols~\cite{Hurley_al02},
Belczynski et al.~\cite{Belczynski_al_startreck}, Yungelson and
Tutukov~\cite{ty02}, De Donder and Vanbeveren~\cite{2004NewAR..48..861D}). A review of applications of the population
synthesis method to various types of astrophysical sources and further
references can be found in~\cite{Popov_Prokhorov04,
  yungelson05b}. Some results of population synthesis
calculations of compact binary mergers carried out by different groups
are presented in Table~\ref{table:mergings}.

\begin{table}
  \renewcommand{\arraystretch}{1.2}
  \caption{Examples of the estimates for Galactic merger rates of
    relativistic binaries calculated under different assumptions on
    the parameters entering population synthesis.}
  \label{table:mergings}
  \centering
  \begin{tabular}{lrrrr}
    \hline \hline
    Authors & Ref. & NS\,+\,NS & NS\,+\,BH & BH\,+\,BH \\
    & & \multicolumn{1}{c}{[yr\super{-1}]} &
    \multicolumn{1}{c}{[yr\super{-1}]} &
    \multicolumn{1}{c}{[yr\super{-1}]} \\
    \hline
    Tutukov and Yungelson (1993) & \cite{ty93b} &
    3~\texttimes~10\super{-4} & 2~\texttimes~10\super{-5} & 1~\texttimes~10\super{-6} \\
    Lipunov et~al.\ (1997) & \cite{LPP97} &
    3~\texttimes~10\super{-5} & 2~\texttimes~10\super{-6} & 3~\texttimes~10\super{-7} \\
    Portegies Zwart and Yungelson (1998) & \cite{py98} &
    2~\texttimes~10\super{-5} & 10\super{-6} \\
    Nelemans et~al.\ (2001) & \cite{nyp01} &
    2~\texttimes~10\super{-5} & 4~\texttimes~10\super{-6} & \\
    Voss and Tauris (2003) & \cite{voss_taurisns03} &
    2~\texttimes~10\super{-6} & 6~\texttimes~10\super{-7} & 10\super{-5} \\
    De Donder and Vanbeveren (2004) & \cite{DeDonder_Vanbeveren04} &
    3~\texttimes~10\super{-3}\,--\,10\super{-5} & 3~\texttimes~10\super{-5} & 0 \\
    O'Shaughnessy et al.\ (2005) & \cite{Oshaughnessy_al05} &
    7~\texttimes~10\super{-6} & 1~\texttimes~10\super{-6} & 1~\texttimes~10\super{-6} \\
    de Freitas Pacheco et al.\ (2006) & \cite{freitas_ns06} &
    2~\texttimes~10\super{-5} \\
    Dominik et al. (2012) & \cite{Dominik_al12} &
24~\texttimes~10\super{-6} & 1.6~\texttimes~10\super{-6} & 8.2~\texttimes~10\super{-6}		\\
    Mennekens and Vanbeveren (2013) & \cite{Mennekens_Vanbeveren13} &
10\super{-7}-10\super{-5} & 10\super{-6}-10\super{-5}& 0 \\
    \hline \hline
  \end{tabular}
  \renewcommand{\arraystretch}{1.0}
\end{table}

Actually, the authors of the studies mentioned in
Table~\ref{table:mergings} make their simulations for a range of
parameters. We list in the table the rates for the models which the
authors themselves consider as ``standard'' or ``preferred'' or
``most probable'', calculated for solar metallicity (or give the ranges, as for 
Brussels code results \cite{Mennekens_Vanbeveren13}). Generally, for the NS\,+\,NS merger rate
Table~\ref{table:mergings} shows the scatter within a factor $\sim$~4,
which may be considered quite reasonable, having in mind the
uncertainties in input parameters. There are several outliers,
\cite{ty93b}, \cite{voss_taurisns03}, and \cite{Mennekens_Vanbeveren13}. The high rate
in~\cite{ty93b} is due to the assumption that kicks to
nascent neutron stars are absent. The low rate in~\cite{voss_taurisns03}
is due to the fact that these authors apply in the common envelope
equation an evolutionary-stage-dependent structural constant
$\lambda$. Their range for $\lambda$ is 0.006\,--\,0.4, to
be compared with the ``standard'' $\lambda=0.5$ applied in most of the
other studies. A low $\lambda$ favours mergers in the first critical
lobe overflow episode and later mergers of the first-born neutron
stars with their non-relativistic companions\epubtkFootnote{Note that
  similar low values of $\lambda$ for $20$ to $50\,M_\odot$ stars were
  obtained also by~\cite{Podsiadlowski_al03}. If confirmed, these
  results may have major impact on the estimates of merger rates for
  relativistic binaries.}. A considerable scatter in the rates of
mergers of systems with BH companions is due, mainly, to
uncertainties in stellar wind mass loss for the most massive
stars. For instance, the implementation of winds in the code used
in~\cite{py98, nyp01} resulted in the absence
of merging BH\,+\,BH systems, while a rather low $\dot{M}$ assumed
in~\cite{voss_taurisns03} produced a high merger rate of BH\,+\,BH
systems.
The results of the Brussels group \cite{DeDonder_Vanbeveren04, Mennekens_Vanbeveren13} differ from \textsc{StarTrack}-code results \cite{Dominik_al12}
and other codes in predicting an insignificant BH-BH merging rate. This is basically due to 
an enhanced mass loss assumed on the red supergiant stage (RSG) of massive star evolution. 
In this scenario, 
unlike, e.g., Voss and Tauris' assumptions~\cite{voss_taurisns03},
the allowance for the enhanced
mass loss at the Luminous Blue Variable (LBV) phase of evolution 
for stars with an initial mass $\gtrsim 30\mbox{\,--\,}40\,M_{\odot}$ leads to a 
significant orbital increase and hence the avoidance of the second
Roche-lobe overflow and spiral-in process in the common envelope,
which completely precludes
the formation of close double BH systems merging within the Hubble time.
The Brussels code also takes into account the time evolution of galactic 
metallicity enrichment by massive single and binary stars. A more detailed 
comparison of different population synthesis results of NS\,+\,NS, NS\,+\,BH and BH\,+\,BH
formation and merging rates can be found in review \cite{Abadie_al10}.

A word of caution should be said here. It is hardly possible to trace
a detailed evolution of each binary, so one usually invokes the
approximate approach to describe the change of evolutionary stages of
the binary components (the so-called evolutionary track), their
interaction, effects of supernovae, etc. Thus, fundamental uncertainties
of stellar evolution mentioned above are complemented with (i)
uncertainties of the scenario and (ii) uncertainties in the
normalisation of the calculations to the real galaxy (such as the
fraction of binaries among all stars, the star formation history,
etc.). The intrinsic uncertainties in the population synthesis results
(for example, in the computed event rates of binary mergers etc.) are
in the best case not less than of the order of factor two or
three. This should always be born in mind when using the population
synthesis calculations. However, we emphasize again the fact that the
double NS merger rate, as inferred from binary pulsar statistics with
account for the double pulsar observations~\cite{Burgay_al03,
 Kalogera_al04, Kim:2013tca}, is very close to the population syntheses 
estimates assuming NS kicks of about (250\,--\,300)~km/s.


==> new_sec_detection_pk.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Notes on the detection rate of compact binary mergings}
%\label{sec:secI:DetectRate}

%\added{REVISED BY KP}

The detection of a gravitational wave signal from merging close
binaries is characterized by the signal-to-noise ratio $S/N$, which
depends on the binary masses, the distance to the binary, the
frequency, and the noise characteristics. A pedagogical derivation of
the signal-to-noise ratio and its discussion for different detectors
is given, for example, in Section~8 of the review~\cite{Grishchuk_al01}.
 
Coalescing binaries emit gravitational wave signals with a well known
time-dependence (waveform) $h(t)$ (see Section~\ref{sec:appA} above). This
allows one to use the technique of matched
filtering~\cite{Thorne87}. The signal-to-noise ratio $S/N$ for a
particular detector, which is characterized by the noise spoectral density 
$S_n(f)$ [$\mathrm{Hz}^{-1/2}]$ or the dimensionless noise
rms amplitude $h_\mathrm{rms}$ at a given frequency $f$, depends
mostly on the ``chirp'' mass of the binary system
$\M=(M_1+M_2)^{-1/5}(M_1M_2)^{3/5}=\mu^{3/5} M^{2/5}$ (here $\mu=M_1M_2/M$ is 
the reduced mass and $M=M_1+M_2$ is the total mass of the system)
and its (luminosity) distance $r$: $S/N\propto \M^{5/6}/r$ \cite{Thorne87, Flanagan_Hughes98}. 
%The simplified version for $S/N$ (\cite{Thorne87}; see
%also~\cite{Flanagan_Hughes98}) reads:
%
%\begin{equation}
%  \frac{S}{N} = 3^{-1/2}\pi^{-2/3} \frac{G^{5/6}}{c^{3/2}}
%  \frac{\M^{5/6}}{r} \frac{f^{-1/6}}{h_\mathrm{rms}(f)}.
%  \label{D:S/N}
%\end{equation}
%
For a given type
of coalescing binaries (NS\,+\,NS, NS\,+\,BH or BH\,+\,BH), the signal-to-noise ratio
will also depend on the frequency of the innermost stable circular orbit
$f_{\mathrm{ISCO}}\sim 1/M$, as well as on the orientation of the binary with respect to the 
given detector and its angular sensitivity (see, e.g.,  
Section~8 in \cite{Grishchuk_al01} and \cite{Sathyaprakash_Schutz09} for more detail). 
Therefore, from the point of view of detection of the specific type of 
coalescing binaries at a pre-requisit signal-to-noise 
ratio level, it is useful to determine the detector's maximum (or `horizon') distance $D_{\mathrm{hor}}$, 
which is calculated for an optimally oriented ('ideal') coalescing binary with a
given chirp mass $\M$.   
For a secure
detection, the $S/N$ ratio is usually raised up to 7\,--\,8 to avoid false
alarms over a period of a year (assuming Gaussian
noise)\epubtkFootnote{If a network of three detectors, such as two
  LIGOs and VIRGO, runs simultaneously, the $S/N$ ratio in an
  individual detector should be $>7/\sqrt{3}\approx 4$)}. This
requirement determines the maximum distance from which an event can be
detected by a given interferometer~\cite{Cutler_Thorne02, Abadie_al10}. The horizon distance 
$D_{\mathrm{hor}}$ of
LIGO~I/VIRGO (advanced LIGO, expected) interferometers for relativistic binary inspirals with
account of the actual noise curve attained in the S5 LIGO scientific run
are given in~\cite{Abadie_al10}: 33(445)~Mpc for
NS\,+\,NS ($1.4\,M_\odot + 1.4\,M_\odot$, $\M_{\mathrm{NS}}=1.22\,M_\odot$), 70(927)~Mpc for NS\,+\,BH
($1.4\,M_\odot + 10\,M_\odot$), and 161(2187)~Mpc for BH\,+\,BH
($10\,M_\odot + 10\,M_\odot$, $\M_{\mathrm{BH}}=8.7\,M_\odot$). The distances increase for a
network of detectors. 


It is worth noting that the dependence of the $S/N$ for different types 
of coalescing binaries on $f_{\mathrm{ISCO}}$ rather slightly (to within 10\%) changes
as $S/N\propto \M^{5/6}$, so, for example, the ratio of BH and NS
detection horizons scales as $S/N$, i.e.  
$D_{hor, BH}/D_{hor, NS}=(\M_{\mathrm{BH}}/\M_{\mathrm{NS}})^{5/6}\approx 5.14$.
This allows us to estimate the relative detection ratio for different 
types of coalescing binaries by a given detector (or a network of detectors).
Indeeed, at a fixed level of $S/N$, the detection volume is proportional to
$D_{\mathrm{hor}}^3$ and therefore it is proportional to $\M^{5/2}$. The detection
rate $\D$ for binaries of a given class (NS\,+\,NS, NS\,+\,BH or BH\,+\,BH) is the
product of their coalescence rate $\R_\mathrm{V}$ with the detector's
horizon volume $\propto \M^{5/2}$ for these binaries.

It is seen from Table~\ref{table:mergings} that the model Galactic
rate $\R_\mathrm{G}$ of NS\,+\,NS coalescences is typically higher than the rate of
NS\,+\,BH and BH\,+\,BH coalescences. However, the BH mass is 
significantly larger than the NS mass. So a binary involving one or
two black holes, placed at the same distance as a NS\,+\,NS binary,
produces a significantly larger amplitude of gravitational waves. With
the given sensitivity of the detector (fixed $S/N$ ratio), a BH\,+\,BH
binary can be seen at a greater distance than a NS\,+\,NS binary. Hence,
the registration volume for such bright binaries is significantly 
larger than the registration volume for relatively weak binaries. The
detection rate of a given detector depends on the interplay between
the coalescence rate and the detector's response to the sources of one
or another kind.

If we assign some characteristic (mean) chirp mass to different types
of double NS and BH systems, the expected ratio of their detection
rates by a given detector is
%
\begin{equation}
  \frac{\D_{\mathrm{BH}}}{\D_{\mathrm{NS}}} =
  \frac{\R_{\mathrm{BH}}}{\R_{\mathrm{NS}}}
  \left( \frac{\M_{\mathrm{BH}}}{\M_{\mathrm{NS}}} \right)^{5/2}\!\!\!\!\!\!\!\!,
\label{DBH/DNS}
\end{equation}
%
where $\D_{\mathrm{BH}}$ and $\D_{\mathrm{NS}}$ refer to BH\,+\,BH and NS\,+\,NS pairs,
respectively. 
Taking $\M_{\mathrm{BH}}=8.7\,M_\odot$ (for $10\,M_\odot + 10\,M_\odot$) 
and $\M_{\mathrm{NS}}=1.22\,M_\odot$ (for $1.4\,M_\odot + 1.4\,M_\odot$), 
Eq.~(\ref{DBH/DNS}) yields
%
\begin{equation}
   \frac{\D_{\mathrm{BH}}}{\D_{\mathrm{NS}}} \approx
   140 \frac{\R_{\mathrm{BH}}}{\R_{\mathrm{NS}}}.
   \label{DBH/DNS.2}
\end{equation}
%
As $\frac{\R_{\mathrm{BH}}}{\R_{\mathrm{NS}}}$ is typically 0.1\,--\,0.01
(see Table~\ref{table:mergings}), this relation suggests that the
registration rate of BH mergers can be \textit{higher} than that of NS
mergers. This estimate is, of course, very rough, but it can serve as
an indication of what one can expect from detailed calculations. We
stress that the effect of an enhanced detection rate of BH binaries is
independent of the desired $S/N$ and other characteristics of the
detector; it was discussed, for example,
in~\cite{ty93b, LPP97, Grishchuk_al01, Dominik_al12}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Note on realistic calculation of the detection rates of
%  binary mergings}

Unlike the ratio of the detection rates, 
the expected value of the detection rate of specific type of compact coalesciong binaries 
by a given detector (network of detectors)
requires detailed evolutionary calculations and the knowledge of the 
actual detector's noise curve, as we discussed
above.
To calculate a realistic detection rate of binary mergers the
distribution of galaxies should be taken into account within the
volume bounded by the detector's horizon (see, for
example, the earlier attempt to take into account only bright galaxies
from Tully's catalog of nearby galaxies in~\cite{Lipunov_al95_gwsky},
and the use of LEDA database of galaxies to estimate the detection
rate of supernova explosions~\cite{Baryshev_Paturel01}). In this context, a
complete study of galaxies within 100~Mpc was done by Kopparapu et al. 
\cite{Kopparapu_al08}. Based on their results, 
Abadie et al. \cite{Abadie_al10} 
derived the approximate formula for the number of the equivalent Milky-Way type galaxies 
within large volumes, which is applicable for distances $\gtrsim 30$~Mpc:
\begin{equation}
\label{sec:det_NG}
N_G(D_{\mathrm{hor}})=\frac{4\pi}{3}\left(\frac{D_{\mathrm{hor}}}{\hbox{Mpc}}\right)^3(0.0116)(2.26)^{-3}\,.
\end{equation}
Here the factor 0.0116 is the local density of the equivalent Milky-Way type
galaxies derived in \cite{Kopparapu_al08}, and the factor 2.26 takes into 
account the reduction in the detector's horizon value when averaging over 
all sky locations and orientations of the binaries. Then the expected detection rate
becomes $\D(D_{\mathrm{hor}})=\R_G\times N_G(D_{\mathrm{hor}})$. 

  
However, not
only the mass and type of a given galaxy, but also the star formation
rate and, better, the history of the star formation rate in that
galaxy are needed to estimate the
expected detection rate $\cal D$ (since the coalescence rate 
of compact binaries in galaxies strongly evolves
with time~\cite{Lipunov_al95_evol, Mennekens_Vanbeveren13, Dominik_al13}).  


So to assess the merger rate from a
large volume based on the Galactic values, the best one can do at
present appears to be using formulas like Eq.~(\ref{sec:det_NG}) or (\ref{R_V}) given
earlier in Section~\ref{sec:ns_freq}. This, however, adds another
factor two of uncertainty in the estimates. Clearly, a more accurate
treatment of the transition from Galactic rates to larger volumes with
an account of the galaxy distribution is very desirable.



To conclude this Section, we will briefly comment on the possible
electromagnetic counterparts of compact binary coalescences.
It is an important issue, since the localization error boxes of NS+NS
coalescences by GE detectors network only are expected to be, 
in the best case, about several square degrees
(see the detailed analysis in \cite{2013arXiv1309.3273R}, as well as 
\cite{Aasi_al13} for discussion of the likely evolution of sensitivity and sky localization of sources for the advanced detectors), which 
is still large for precise astronomical identification. Any associated electromagnetic signal can greatly help to pinpoint the source.
Double NS
mergings are the most likely progenitors of short gamma-ray bursts
(\cite{Nakar07,FongBerger13} and references therein). Indeed, 
recently, a short-hard GRB~130603B was found to be followed by a 
rapidly fading  IR afterglow
\cite{Berger_al13}, which is most likely due to `macronova' or
`kilonova' produced by decaying radioactive heavy elements expelled during a double
NS merging \cite{Li_Paczynski98, Rosswog05, Metzger_al10, Hotokezaka_al13, 2014MNRAS.tmp..182G}. Detection of
electromagnetic counterparts to GW signals from coalescing binaries is an
essential part of the strategy of the forthcoming advanced LIGO/VIRGO
observations \cite{2014MNRAS.437..649S}. Different aspects of this multi-messenger GW astronomy are further 
discussed in papers \cite{2013PhRvD..88d3011P,
2013ApJ...767..124N,2013arXiv1309.1554K, Aasi_al13,2013arXiv1312.5133M}, etc.

